Efficient Irregular Wavefront Propagation Algorithms on Hybrid CPU-GPU Machines

In this paper, we address the problem of efficient execution of a computation pattern, referred to here as the irregular wavefront propagation pattern (IWPP), on hybrid systems with multiple CPUs and GPUs. The IWPP is common in several image processing operations. In the IWPP, data elements in the wavefront propagate waves to their neighboring elements on a grid if a propagation condition is satisfied. Elements receiving the propagated waves become part of the wavefront. This pattern results in irregular data accesses and computations. We develop and evaluate strategies for efficient computation and propagation of wavefronts using a multi-level queue structure. This queue structure improves the utilization of fast memories in a GPU and reduces synchronization overheads. We also develop a tile-based parallelization strategy to support execution on multiple CPUs and GPUs. We evaluate our approaches on a state-of-the-art GPU accelerated machine (equipped with 3 GPUs and 2 multicore CPUs) using the IWPP implementations of two widely used image processing operations: morphological reconstruction and euclidean distance transform. Our results show significant performance improvements on GPUs. The use of multiple CPUs and GPUs cooperatively attains speedups of 50x and 85x with respect to single core CPU executions for morphological reconstruction and euclidean distance transform, respectively.

==> background.tex <==
\section{Motivation} \label{sec:motivation}
%
Our work is primarily motivated by the computational requirements of biomedical imaging 
studies involving digital microscopy images. As part of the work done at the In Silico 
Brain Tumor Research Center, our group has developed image analysis pipelines 
to extract and classify morphology and texture information from high resolution 
microscopy images, with the objective of exploring correlations between tissue morphology
features, genomic signatures, and clinical data. These pipelines share a common set of 
cascaded stages, including: 1) image preprocessing tasks such as color
normalization, 2) segmentation of micro-anatomic objects and regions of
interest such as cells and nuclei, 3) characterization of the shape and texture
features of the segmented objects, and 4) machine-learning methods that integrate
information from features to classify the objects. Each stage consists of a
sequence of operations as nested pipelines in the overall analysis pipeline. 
In terms of computational cost, preprocessing and classification stages are
inexpensive relative to segmentation and feature extraction. 
The segmentation and feature computation stages operate on $10^{5}$ to $10^{7}$ 
cells and nuclei in an image of size $10^{5}$ by $10^{5}$ pixels.  
The classification stage as required by the scientific application includes
significant data reduction prior to the actual classification operation which 
decreases computational requirements.

Our performance optimization efforts therefore have been focused on the segmentation
and feature computation stages. The operations in these stages can be
roughly grouped into those that are spatially-independent,
iterative and non-iterative neighborhood-based, and object-based.  As many of
these operations are data parallel and computationally intensive, we are in the
process of implementing parallel and GPU versions to support execution on 
high performance computing systems consisting of nodes with multi-core 
CPUs and multiple GPUs. In an earlier work~\cite{Teodoro-IPDPS2012}, we 
developed performance-aware scheduling techniques to efficiently map 
feature computation operations to multiple devices (i.e., CPUs 
and GPUs) in a distributed memory system in order to maximize computation throughput.

The segmentation stage has proven to be more complex. The general approach in
the segmentation stage for nuclei is to use morphological reconstruction (one
of our use case algorithms to employ wavefront propagation computation) to
identify candidate objects, separate overlapping objects using watershed
segmentation, and then heuristically filter out the candidates that are
unlikely to be nuclei based on object characteristics.  The actual pipeline
consists of over 20 component operations, some as compound operations
themselves, forming a directed acyclic dependency graph. Many of these
operations have existing GPU implementations in OpenCV~\cite{opencv_library} or
are easy to port to GPU. Our measurements of the time cost of the individual
operations in the pipeline, weighted by the number of invocations of each
operation, showed that the morphological reconstruction, watershed
segmentation, and distance transform are the most expensive operations on CPU
in decreasing order. We were able to identify an efficient GPU-based watershed
segmentation implementation~\cite{Korbes:2011:AWP:2023043.2023072}, but the
remaining two operations require new GPU implementations and optimizations. 

The morphological reconstruction operation is a good candidate for GPU
acceleration, since it is invoked in many places in the segmentation stage.  It
can be used to establish a local threshold around a target object --- the
object can then be obtained through a subtraction of the reconstructed image
from the original.  This is how candidate nuclei are detected in image analysis
pipelines.  It is also used as component operations in other operations,
including hole filling and seeded object selection in binary images, and
regional extrema detection and noise removal in gray scale images. Morphological
reconstruction is a powerful method. In fact, morphological reconstruction is
utilized in a number of image processing operations for its ability to select
objects based on seeded points, to remove noise, and to establish local
thresholds. A survey of MATLAB functions showed that morphological
reconstruction is used as an internal operation for at least nine different
functions\footnote{MATLAB function utilizing morphological reconstruction
internally include imregionalmin, imregionalmax, imhmin, imhmax, imextendedmin,
imextendedmax, imclearborder, imimposemin, imfill}. Vincent, in his seminal
paper on morphological gray scale
reconstruction~\cite{Vincent93morphologicalgrayscale}, outlines several
applications: select objects with desired size and shape by using morphological
open to seed the objects of sufficient size and shape, followed by
morphological reconstruction to extract selected objects from the original
image, and optionally subtract the results from the original image if the small
objects are desired; determine regional minima and maxima, which are regions
surround by pixels with higher or lower values, respectively; identify the
h-domes, which represent light objects with a maximum intensity variation of h,
regardless of size or shape; condition image and generate markers for watershed
segmentation. 

The distance transform operation, on the other hand, is used in our pipeline as
a pre-process step to the separation of overlapping objects using watershed.
The distance transform is computed on top of a binary mask image to convert it
into a gray level image, which is suitable for watershed computation. The
main commonality among morphological reconstruction and distance transform
operations, which motivated this work, is that both can be efficiently computed
using the wavefront propagation
framework~\cite{Vincent93morphologicalgrayscale}. Therefore, instead
individually porting each of the operations for GPUs, our effort focused on
building a more generic framework that would allow for implementing a class of
applications that include at least morphological algorithms based on
neighborhood operators for hybrid CPU---GPU equipped systems.

%Jivet et al. also reported using morphological reconstruction
%during image contrast enhancement~\cite{Jivet:2008:ICE:1482247.1482253}. A well
%optimized GPU implementation of morphological reconstruction is therefore
%beneficial for our segmentation pipeline as well as other image analysis
%implementations in general.

%In the rest of 
%the paper we present an overview of the morphological reconstruction 
%operation, a GPU-enabled implementation of the operation, and an experimental 
%evaluation of the implementation's performance on a state-of-the-art GPU 
%system. 





    



 


==> implementation.tex <==
\subsection{Implementation} \label{sec:gpufphr}
%
This section describes the details of FH\_GPU implementation and the
optimizations for efficient execution on a GPU.  The raster scan phase of
FH\_GPU is presented in Section~\ref{sec:antiraster}.  This first stage of the
algorithm  has a more regular data access and processing pattern, since that
computation is applied to the entire input image.  The queue-based pixel
computation phase is described in Section~\ref{sec:queuebasedgpu}.  The
computation structure of this phase, unlike the first phase, is irregular,
because  only active pixels, which are sparsely and irregularly spread across
the image, are processed.  

%
\subsubsection{Raster Scan Phase} \label{sec:antiraster}
%
The GPU version of the raster scan phase extended from the implementation by
Karas~\cite{DBLP:conf/memics/Karas10}.  We have made several changes to the
original implementation to improve performance in  our use cases: (1) we have
templated our implementation to support binary images as well as gray scale
images with integer and floating point data types; (2) we have optimized the
implementation and multi-threaded execution for 2-dimensional images-- the
original implementation was designed for 3-dimensional images. This
modification allows us to specialize the Y-direction propagation during the scans; and (3) we have tuned the shared memory utilization to minimize
communication between memory hierarchies.  

The raster and anti-raster scans are implemented in four GPU kernels:
y\_Forward, x\_Forward, y\_Backward, and x\_Backward. The y\_Forward kernel is
executed by $N_x$ threads in the GPU, where $N_x$ is the size of a block of
columns of the images.  The input marker and mask images as well as the
{\em global change variable}, which keeps track of pixel value changes, are
stored in the GPU global memory. Shared memory is used to improve data access.
The y\_Forward kernel loads 2 rows of the marker and mask images into the GPU
shared memory and $N_x$ threads in parallel updates the pixel values.  The
kernel iterates over all rows in one kernel invocation.

The x\_Forward kernel is executed using $N_{xx}$ by $N_{xy}$ threads. The thread block size is
determined by the available shared memory size of the GPU.  During execution,
the kernel first loads $N_{xy} \times N_{xy}$ pixels from the marker and mask images
into the shared memory using all $N_{xx}$ by $N_{xy}$ threads, then $N_{xy}$ threads update the values in the rows, one
thread per row, concurrently.  $N_{xy}$ is chosen as a multiple of 
the warp size of the GPU's symmetric multiprocessor in ordre to maximize coalesced global memory access and avoid shared memory bank conflicts, while $N_{xx}$ is chosen to be small (e.g., four
threads) to maximize the fraction of threads performing computation.
At the end of each iteration, the data is copied back to the GPU global memory.   
 
The x\_Backward and y\_Backward kernels for anti-raster scans are the same as
the x\_Forward and y\_Forward kernels, respectively, except for the fact that
they scan the images in the anti-raster direction. 

The scans are repeated until a predetermined iteration count is reached, or the stability 
is achieved as in the sequential reconstruction algorithm. At the end of each iteration, 
the global change variable is checked to determine if the stability has been achieved.    
%
\subsubsection{Queue-based Computation Phase} \label{sec:queuebasedgpu}
%
In this section, first the parallelization strategy for the queue-based computation 
phase is presented. This is followed by the description of the implementation of the 
parallel queue structure employed in the computation. 
%
\paragraph{Parallelization Strategy}
After the raster scan phase, {\em active pixels}, which are the pixels whose 
values could be propagated to neighbor pixels in the next iteration of 
the algorithm, are put into a global queue for computation. The global queued is then 
equally partitioned into a number of smaller queues. Each of these queues is assigned 
to a GPU thread block. Each block can carry out computations independent 
of the other blocks. This 
partitioning and mapping strategy reduces the communication and synchronization 
costs to access the global queue and ensure consistency of the queue. With this 
strategy, it is not necessary to 
employ expensive inter-block synchronizations~\cite{DBLP:conf/ipps/XiaoF10} or
continuously utilize system level $Memory\ Fence\ Operations$ to assert
queue consistency across GPU multi-processors.

Two levels of parallelism can be implemented in the queue-based computation
performed by each thread of block: (i)~pixel level parallelism which allows
pixels queued for computation to be independently processed; and (ii)~the
neighborhood level parallelism that performs the concurrent evaluation of a
pixel neighborhood. The pixel and neighborhood level parallelism correspond to
the parallel loops shown in Lines 20 and 21 from Algorithm~\ref{alg:fhgpu},
respectively. The parallelism in both cases, however, is available at the cost
of dealing with potential race conditions that may occur when a pixel is
updated concurrently.  

\begin{algorithm}
\caption{GPU-based queue propagation phase}
\label{alg:queuephasegpu}
\begin{algorithmic}[1]
\STATE\{Split initial queue equally among thread blocks\}
\WHILE{queue\_empty() = false}
%	\STATE in\_size=queue.size()
%	\FOR{$i=tid\_in\_block; i < in\_size; i+=block\_size$} 
 	\WHILE{$(p = dequeue(...)) != EMPTY$} {\bf in parallel}
%		\STATE {}
		\FORALL{$q \in N_{G}(p)$} 
			\IF{$J(q) < J(p)$ and $I(q) \neq J(q)$}
				\STATE $oldval = atomicMax(\&J(q), min\{J(p),I(q)\})$
				\IF{$oldval <  min\{J(p),I(q)\}$}
					\STATE queue\_add(q)
				\ENDIF
			\ENDIF
		\ENDFOR
	\ENDWHILE
	\IF{$tid=0$}
		\STATE{queue\_swap\_in\_out()}
	\ENDIF
	\STATE $\_\_syncthreads()$
	\STATE $\_\_threadfence\_block()$
\ENDWHILE
\end{algorithmic}
\end{algorithm}

During execution, a {\em value max} operation is performed on the value of the
current pixel being processed ($p$) and that of each pixel in the neighborhood
($q \in N_G(p)$) --- limited by a fixed mask value $I(q)$. To correctly perform
this computation, atomicity is required in the maximum and update operations.
This can only be achieved at the cost of extra synchronization overheads.  The
use of atomic CAS operations is sufficient to solve this race condition.  The
efficiency of atomic operations in GPUs have been significantly improved in the
last generation of NVidia GPUs (Fermi)~\cite{citeulike:8927897} because of the
use of cache memory. Atomic operations, however, still are more efficient in
cases where threads do not concurrently try to update the same memory address.
When multiple threads attempt to update the same memory location, the threads
are serialized in order to ensure correct execution. As a result, the number of
operations successfully performed per cycle is drastically
reduced~\cite{citeulike:8927897}. 

To lessen the impact of the potential serial execution, our GPU parallelization
employs the pixel level parallelism only. The neighborhood level parallelism is
problematic in this case because the concurrent processing and updating of
pixels in a given neighborhood likely affect one another,
since the pixels are located in the same region of the image. Unlike
traditional graph computing algorithms (e.g., Breadth-First
Search~\cite{Hong:2011:ACG:1941553.1941590,Luo:2010:EGI:1837274.1837289}), the
lack of parallelism in neighborhood processing does not result in load
imbalance in the overall execution, because all pixels have the same number of
neighbors which is defined by the structuring element $G$.

The GPU-based implementation of the queue propagation operation is presented in
Algorithm~\ref{alg:queuephasegpu}. After splitting the initial queue, each
block of threads enters into a loop in which pixels are dequeued in parallel
and processed, and new pixels may be added to the local queue as needed.  This
process continues until the queue is empty. Within each loop, the pixels queued
in last iteration are uniformly divided among the threads in the block and
processed in parallel (Lines 3---8 in Algorithm~\ref{alg:queuephasegpu}). The
value of each queued pixel $p$ is compared to every pixel $q$ in the
neighborhood of pixel $p$.  An atomic maximum operation is performed when a
neighbor pixel $q$ should be updated.  The value of pixel $q$ before the
maximum operation is returned ($oldval$), and used to determine whether the
pixel's value has really been changed (Line 7 in
Algorithm~\ref{alg:queuephasegpu}). This step is necessary because there is a
chance that another thread might have changed the value of $q$ between the time
the pixel's value is read to perform the update test and the time that the
atomic operation is performed (Lines 5 and 6 in
Algorithm~\ref{alg:queuephasegpu}). If the maximum operation performed by the
current thread has changed the value of pixel $q$, $q$ is added to the queue
for processing in the next iteration of the loop. Even with this control, it
may happen that between the test in line 7 and the addition to the queue, the
pixel $q$ may have been modified again. In this case, $q$ is added multiple
times to the queue, and although it impacts the performance, the correctness of
the algorithm is not affected.

After computing pixels from the last iteration, pixels that are added to the queue 
in the current iteration are made available for the next iteration, and all writes
performed by threads in a block are guarantee to be consistent (Lines 9 to 12 in the 
algorithm).
As described in the next section, the choice to process pixels in rounds,
instead of making each pixel inserted into the queue immediately accessible, is 
made in our design to implement a queue with very efficient read performance (dequeue 
performance) and with low synchronization costs to provide consistency among threads 
when multiple threads read from and write to the queue.
%
\paragraph{Parallel Queue Implementation and Management}
\label{sec:parqueue}
%
The parallel queue is a core data structure employed by FH\_GPU. 
The queue is used to
store and retrieve pixel information associated with computation.  An efficient
parallel queue for GPUs is a challenging 
problem~\cite{Hong:2011:ACG:1941553.1941590,DBLP:conf/memics/Karas10,Luo:2010:EGI:1837274.1837289}
due to the sequential and irregular nature of accesses.

A straight forward implementation of a queue (named Na\"{\i}ve here), as
presented by Hong et al.~\cite{Hong:2011:ACG:1941553.1941590}, could be done by employing
an array to store items in sequence and using atomic additions to calculate the
position where the item should be inserted, as presented in the
code bellow.

\begin{verbatim}
  AddQueue(int* q_idx, type_t* q, type_t item) {
    int old_idx = AtomicAdd(q_idx, 1);
    q[old_idx] = item; }
\end{verbatim}

Hong et al. stated that this solution worked well for their use case. The use
of atomic operations, however, is very inefficient when the queue is heavily
employed as in our algorithm. Moreover, a single queue that is shared among all
thread blocks introduces additional overheads to guarantee data consistency
across the entire device. It may also require expensive inter-block
synchronization primitives~\cite{DBLP:conf/ipps/XiaoF10} to synchronize threads
from multiple block that are not standard methods supported by CUDA.

\begin{figure}[htb!]
\begin{center}
\includegraphics[width=0.7\textwidth]{images/queue}
\vspace*{-2ex}
\caption{Multi-level parallel queue.}
\vspace*{-2ex}
\label{fig:parallelqueue}
\end{center}
\end{figure}

Therefore, we have designed a parallel queue that operates
independently in a per thread block basis to avoid inter-block communication, and is
built with a cascade of storage levels in order to exploit the GPU fast memories 
for fast write and read accesses. The parallel queue (depicted in
Figure~\ref{fig:parallelqueue}) is constructed in
multiple-levels:(i)~Per-Thread queues (TQ) which are very small queues
private to each thread, residing in the shared memory; (ii)~Block Level Queue
(BQ) which is also in the shared memory, but is larger than TQ. Write operations 
to the block level queue are performed in thread warp-basis; and (iii)
Global Block Level Queue (GBQ) which is the largest queue and uses the global memory 
of the GPU to
accumulate data stored in BQ when the size of BQ exceeds the shared memory size.

The use of multiple levels of queues improves the scalability of the implementation,
since portions of the parallel queue are utilized independently and the fast memories
are employed more effectively. In our queue implementation, each thread maintains an 
independent queue (TQ) that does not require any synchronization to be performed. 
In this way threads can efficiently store pixels from a given neighborhood in the 
queue for computation. Whenever this level of queue is full, it is necessary
to perform a warp level communication to aggregate the items stored in local
queues and write them to BQ. In this phase, a parallel thread warp
prefix-sum is performed to compute the total number of items queued in 
individual TQs. A single shared memory atomic operation is performed at the Block Level
Queue to identify the position where the warp of threads should write their
data. This position is returned, and the warp of threads write their local
queues to BQ.

Whenever a BQ is full, the threads in the corresponding thread block are
synchronized.  The current size of the queue is used in a single operation to
calculate the offset in GBQ from which the BQ should be stored. After this
step, all the threads in the thread block work collaboratively to copy in
parallel the contents of QB to GBQ. This data transfer operation is able to
achieve high throughput, because the memory accesses are coalesced. It should
be noted that, in all levels of the parallel queue, an array is used to hold
the queue content. While the contents of TQ and BQ are copied to the lower
level queues when full, GBQ does not have a lower level queue to which its
content can be copied. In the current implementation, the size of GBQ is
initialized with a fixed tunable memory space. If the limit of GBQ is reached
during an iteration of the algorithm, excess pixels are dropped and not stored.
The GPU method returns a boolean value to CPU to indicate that some pixels have
been dropped during the execution of the method kernel.  In that case, the
algorithm has to be re-executed, but using the output of the previous execution
as input, because this output already holds a partial solution of the problem.
Hence, recomputing using the output of the previous step as input will result
in the same solution as if the execution was carried out in a single step. 

While adding new items to the queue requires a number of operations to
guarantee consistency, the read operations in our application can be
performed without introducing synchronization. This is possible by partitioning
input data elements statically among threads, which keep consuming
the data elements until all items are computed. The drawbacks of a
static partition of the queue and work within a loop iteration is minimum 
in our application,  
because the computation cost of queued pixels is similar; only a minor load
imbalance is introduced with this solution. Moreover, queued pixels are repartitioned
at each new iteration of the loop. A high level description of the $dequeue$
function is presented bellow. 
In this function, the value of the item is initialized to a default
code corresponding to an empty queue. Then, the queue index corresponding to the
next item to be returned for that particular thread is calculated, based on the
size of the thread block ($block\_size$), the number of iterations already
computed by this thread warp ($iter$), and the identifier of that thread in the
block.

\begin{verbatim}
type_t DeQueue(int q_size, type_t* q, int iter) {
  type_t item = QUEUE_EMPTY;
  queue_idx = tid_in_block + iter * block_size;
  if(queue_idx < q_size){
     type_t item = q[queue_idx];
  }
  return item; }
\end{verbatim}

%\subsection{Potential optimizations}
%
%\begin{itemize}
%	\item Modify the number of thread in a thread block when the queue is
%small, or exploit the neighborhood parallelism on that case;
%
%	\item Read multiple pixels from the queue at once (chunk)
%
%	\item Perform Load balancing among blocks if queue sizes are too different;
%\end{itemize}


==> model.tex <==
\section{Performance Model} \label{sec:model}
%
We present an analytical model to assess the performance of the
scheduling and optimizations proposed in this work. The main intention
of this framework is to provide a set of tools that could be used to
estimate the performance impact of the proposed optimizations for a
given set of tasks, presumably of a candidate application for
implementation in our execution model, without necessarily
implementing the application. Moreover, this framework may be used to
analyze the impact various aspects, e.g. the error in speedup
estimation, to the scheduling policies used, as well as it formalizes
the scheduling problem.

The task scheduling problem we study in this work is dynamic in the
sense that tasks may be created during the execution, at times unknown
prior to the execution. Thus, off-line scheduling is not possible and
proper mapping decisions must be carried on-the-fly as tasks become
available.  Most of the framework constructed is common for all
proposed scheduling policies, except for the final decision of what
task is chosen for execution at each mapping time.

Let $T$ be the set of all tasks $w_i$, $1 \le i \le m$, computed by an
application during the execution, each of them created at a timestamp $c_i$ not
known prior to execution.  Assume that there is no preemption in a task
execution; each task is assigned to a single heterogeneous processor $p_j \in
p_1\dots p_n$; and, the estimated execution time of a given task $w_i$ using
processor $p_j$ is denoted as $e_{ij}$. Further, let $T^t$ be the set of tasks
created before or on timestamp $t$, which have not been scheduled for
execution.  The subset of tasks mapped to a given processor $p_j$ on or before
time $t$ is expressed as $PT_j^t$, the schedule for all processor at time $t$
as $PT^t$, and $idle_{ij}$ is the idle time elapsed between $w_i$ start time and the
end of the last task assigned to processor $p_j$.  Notice that $idle_{ij}$ may
represent several aspects as scheduling overhead, data transfer times required
to start a task, insufficient parallelism, or it could be also ignored for
simplified analysis. Further, $F(PT^t_j)$, the predicted finish time of machine
$j$ for tasks assigned on or before time $t$ may be calculated as:

\begin{equation}
F(PT^t_j) = \sum_{k \in PT_j^t} (e_{kj} + idle_{kj})
\end{equation}

In our approach, the mapping of tasks to processors is demand-driven and a
single task is assigned to a processor whenever at least one processor is
available ($\tau(PT^t) = \min_{1\le j \le n} F(PT^t_j)$), and there are tasks to be
scheduled ($T^t \neq \emptyset$). Additionally, the next non-empty set of
tasks on or after timestamp $t$ is $\zeta(t)$:

\begin{equation}
  \zeta(t) = \left\{ 
  \begin{array}{l l}
    t 		& \quad \text{if $T^t \neq \emptyset$}\\
    min_{1\le i\le m}(c_i\ |\ c_i > t) 	& \quad \text{otherwise}\\
  \end{array} \right.
\end{equation}

Thus, the next mapping time on or after a given timestamp $t$ may be calculated
as $\beta(t) = max(\tau(PT^t), \zeta(t))$. The processor to receive the next
task at a given mapping time $t'=\beta(t)$ is that processor with smallest predicted
finish time at timestamp $t'$ ($\phi(t') = \underset{1 \le j \le
n}{\operatorname{argmin}}\ F(PT^{t'}_j)$). Further, we define the function
$\vartheta(t)$ that calculates the mapping of a single task at time $t$:

\begin{equation}
\vartheta(t) = \beta(\tau(PT_{\phi(t)}^t \leftarrow select(T^{t}, POLICY)))
\label{eq:mapping}
\end{equation}

%\begin{equation}
%\vartheta(t) = \beta(\tau(PT_{\phi(\beta(t))} \leftarrow select(T^{\beta(t)}, POLICY)))
%\label{eq:mapping}
%\end{equation}

The $\vartheta(t)$ first calculates the set of tasks ready to execute at the
mapping time $t$ ($T^{t}$), selects one task according to the scheduling policy
chosen, e.g. FCFS or PRIORITY, and assigns that task to the processor with
minimum finish time at time $t$ ($\phi(t)$). After the mapping is performed, the
timestamp of the next mapping is computed as a result.

In practice, the overall schedule is calculated as a sequence of $m$ mappings,
which are dynamically calculated based on the previous mappings results. Thus,
the global schedule may computed recursively using function $Z(m)$ that
utilizes $\vartheta(t)$ defined before to compute every single mapping.  As
shown bellow, the result of each $Z(N)$ is the timestamp of the next
mapping ($N + 1$), which is recursively given as input to $\vartheta(t)$.

\begin{equation}
  Z(m) = \left\{ 
  \begin{array}{l l}
    \beta(0) 		& \quad \text{if $ m = 0$}\\
    \vartheta(Z(m-1))	& \quad \text{otherwise}\\
  \end{array} \right.
%\vartheta(N) = PT_{\phi(\beta(t))} \leftarrow select(T^{\beta(t)}), t'=\beta(t)
\label{eq:mapping2}
\end{equation}

After $m$ mappings, the makespan may be calculated as the $max_{1\le j \le n}
F_j(Z(m))$, or optionally as $max_{1\le j \le n} F_j(\infty)$.  The performance
of the scheduling policies in this framework are differentiated through the
$select$ function implemented by each of them. While FCFS chooses the task with
smallest creation time $c_i \in T^{\beta(t)}$, PRIORITY orders the task in
$T^{\beta(t)}$ according to the expected speedup to select that task with
highest speedups to the GPU and smallest speedup to the CPU. 
%As discussed,
%these tools are important as one would be able to estimate the effects of the
%proposed scheduling techniques with minor implementation effort, based on the
%tasks' profile of an application. 


